CREval: An Automated Interpretable Evaluation for Creative Image Manipulation under Complex Instructions

Instruction-based multimodal image manipulation has recently made rapid progress. However, existing evaluation methods lack a systematic and human-aligned framework for assessing model performance on complex and creative editing tasks. To address this gap, we propose CREval, a fully automated question-answer (QA)-based evaluation pipeline that overcomes the incompleteness and poor interpretability of opaque Multimodal Large Language Models (MLLMs) scoring. Simultaneously, we introduce CREval-Bench, a comprehensive benchmark specifically designed for creative image manipulation under complex instructions. CREval-Bench covers three categories and nine creative dimensions, comprising over 800 editing samples and 13K evaluation queries. Leveraging this pipeline and benchmark, we systematically evaluate a diverse set of state-of-the-art open and closed-source models. The results reveal that while closed-source models generally outperform open-source ones on complex and creative tasks, all models still struggle to complete such edits effectively. In addition, user studies demonstrate strong consistency between CREval's automated metrics and human judgments. Therefore, CREval provides a reliable foundation for evaluating image editing models on complex and creative image manipulation tasks, and highlights key challenges and opportunities for future research.

==> rebuttal_tables/cost_compare.tex <==
% \begin{table}[h]
    \vspace{-1.5em}
    \centering
    % 调整标题上方间距（图片与标题间），负值收紧
    \setlength{\abovecaptionskip}{-0cm} 
    % % 调整标题下方间距（标题与正文间），负值收紧
    \setlength{\belowcaptionskip}{0.1cm} 
    \caption{Cost Comparison.}
    % \renewcommand{\arraystretch}{1.1}
    \resizebox{0.25\textwidth}{!}{
        \begin{tabular}{ccc}
             \noalign{\hrule height 1.5pt}
             Methods & CREval & VIEScore \\
             \hline
             
             Time &  &    \\
             Token & 8.74M & 1.93M \\

             % \rowcolor{grey!20} Human Consistency &  &  &  &  &  &  & - \\

             \noalign{\hrule height 1.5pt}
             
        \end{tabular}
    }
    \label{tab:cost_comparation}
\vspace{-1.5em}
% \end{table}

==> rebuttal_tables/evaluate.tex <==
\begin{table}[t]
    \centering
    % 调整标题上方间距（图片与标题间），负值收紧
    \setlength{\abovecaptionskip}{0.1cm} 
    % 调整标题下方间距（标题与正文间），负值收紧
    \setlength{\belowcaptionskip}{-0cm} 
    \caption{Experimental results on different evaluators.}
    % \renewcommand{\arraystretch}{1.1}
    \resizebox{0.45\textwidth}{!}{
        \begin{tabular}{cccccc}
             \noalign{\hrule height 1.5pt}
             Evaluator & Qwen3-VL & GPT4o & Seed-1.6  & Human \\
             \hline

             FLUX.1-Kontext [dev] & 80.38 & 75.05 & 80.39 & 47.77 \\
             GPT-Image-1 & 83.15 & 78.01 &  80.99 & 59.89 \\
             Qwen-Image-Edit & 83.02 & 79.18 & 81.39 & 61.81\\
             Gemini 2.5 flash image & \textcolor{red}{87.14} &  \textcolor{red}{81.78} & \textcolor{red}{85.76} & \textcolor{red}{62.70}\\

             % \rowcolor{grey!20} Human Consistency &  &  &  &  &  &  & - \\

             \noalign{\hrule height 1.5pt}
             
        \end{tabular}
    }
    \label{tab:evaluation}
\vspace{-2.8em}
\end{table}

==> rebuttal_tables/weight.tex <==
\begin{table}[h]
    \vspace{-1.5em}
    \centering
    % 调整标题上方间距（图片与标题间），负值收紧
    \setlength{\abovecaptionskip}{-0cm} 
    % 调整标题下方间距（标题与正文间），负值收紧
    \setlength{\belowcaptionskip}{0.15cm} 
    \caption{Comparison of weight ratios.}
    % \renewcommand{\arraystretch}{1.1}
    \resizebox{0.3\textwidth}{!}{
        \begin{tabular}{ccccc}
             \noalign{\hrule height 1.5pt}
             Methods & 1:1:1 & 2:4:4 & 4:2:4 & 4:4:2  \\
             \hline
             
             Bagel & 70.69 & 69.17 & 74.09 & 68.82   \\
             OmniGen2 & 70.69 & 70.51 & 73.38 & 68.17   \\
             Qwen-Image-Edit & 81.53 & 80.67 & 84.13 & 79.78   \\
             GPT-Image-1 & 81.01 & 79.54 & 84.52 & 78.97   \\
             Gemini 2.5 & 82.85 & 82.74 & 84.46 & 81.34   \\

             % \rowcolor{grey!20} Human Consistency &  &  &  &  &  &  & - \\

             \noalign{\hrule height 1.5pt}
             
        \end{tabular}
    }
    \label{tab:weight}
\vspace{-1.5em}
\end{table}

==> table/closed-models.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.1}
    \caption{experiment result}
    \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{c|c|c|cccc}
            \noalign{\hrule height 1.5pt}
            
            \multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Dimension}} & \multirow{2}{*}{\textbf{Metric}} & 
            \multicolumn{4}{c}{\textbf{Closed-Source Models}} \\
            \cline{4-7}

            & & &
            \textbf{GPT-Image-1} & \textbf{\makecell[t]{seedream \\ 4.0}} & \textbf{\makecell[t]{Gemini 2.5 Flash Image \\ (Nano Banana)}} & \textbf{\makecell[t]{FLUX.1 \\ Kontext[pro]}}
            \\
            \hline
            

            \multirow{13}{*}{\rotatebox{90}{\textbf{Customization}}} 
            & \multirow{4}{*}{\makecell{Derivative \\ Character}} & IF & 88.88 & 00.00 &  &    \\
            % \cline{3-11}
            & & VC & 88.88 &  &  &     \\
            % \cline{3-11}
            & & VQ & 88.88 &  &  &   \\
            % \cline{3-11}
            & & avg & 88.88 &  &  &     \\
            \cline{2-7}
            
            & \multirow{4}{*}{\makecell{Reimagined \\ Representations}} & IF & 00.00 &  &  &   \\
            % \cline{3-11}
            & & VC & 00.00 &  &  &    \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &   \\
            % \cline{3-11}
            & & avg & 00.00 &  &  &   \\
            \cline{2-7}
            
            & \multirow{4}{*}{\makecell{Surreal \\ Fantasy}} & IF & 00.00   &  &  & \\
            % \cline{3-11}
            & & VC & 88.88 &  &  &   \\
            % \cline{3-11}
            & & VQ & 88.88 &  &  &   \\
            % \cline{3-11}
            & & avg & 88.88 &  &  &   \\
            \cline{2-7}
            
            & \textbf{Average} & - & 88.88 &  &  &   \\
            % \hline
            \noalign{\hrule height 1.5pt}
            
            
            % Contextualization任务组
            \multirow{13}{*}{\rotatebox{90}{\textbf{Contextualization}}} 
            & \multirow{4}{*}{\makecell{Containerized \\ scenario}} & IF & 00.00 &  &  &   \\
            % \cline{3-11}
            & & VC & 00.00 &  & &    \\
            % \cline{3-11}
            & & VQ & 00.00 &  & &  \\
            % \cline{3-11}
            & & avg & 00.00 &  & &  \\
            \cline{2-7}
            
            & \multirow{4}{*}{\makecell{Commercial \\ design}} & IF & 00.00   &  &  & \\
            % \cline{3-11}
            & & VC & 00.00 &  &  &   \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &   \\
            % \cline{3-11}
            & & avg & 00.00   &  &  & \\
            \cline{2-7}
            
            & \multirow{4}{*}{\makecell{Informationization\& \\ Narrative Expression}} & IF & 00.00 &  &   & \\
            % \cline{3-11}
            & & VC & 00.00 &  &  &   \\
            % \cline{3-11}
            & & VQ & 00.00 &  &   & \\
            % \cline{3-11}
            & & avg & 00.00 &  &   & \\
            \cline{2-7}
            
            & \textbf{Average} & - & 00.00 &  &  & \\
            \noalign{\hrule height 1.5pt}
            
            % Stylization
            \multirow{13}{*}{\rotatebox{90}{\textbf{Stylization}}} 
            & \multirow{4}{*}{\makecell{Artistic Style \\ Transformation}} & IF & 88.88 &  &   & \\
            % \cline{3-11}
            & & VC & 88.88 &  &    & \\
            % \cline{3-11}
            & & VQ & 88.88 &  &  & \\
            % \cline{3-11}
            & & avg & 88.88 &  &  & \\
            \cline{2-7}
            
            & \multirow{4}{*}{\makecell{Identity\&Cultural \\ Transformation}} & IF & 00.00 &  &   & \\
            % \cline{3-11}
            & & VC & 00.99 &  &  &   \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &   \\
            % \cline{3-11}
            & & avg & 00.00   &  &  & \\
            \cline{2-7}
            
            & \multirow{4}{*}{\makecell{Material \\ Transformation}} & IF & 00.00 &  &  &   \\
            % \cline{3-11}
            & & VC & 00.00 &  &  &   \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &   \\
            % \cline{3-11}
            & & avg & 00.00 &  &  &   \\
            \cline{2-7}

            & \textbf{Average} & - & 00.00 &  &   & \\
            \hline
            
            & \multicolumn{2}{c|}{\textbf{Overall Average}} & 00.00   &  &  &   \\
            \noalign{\hrule height 1.5pt}
        \end{tabular}
    }
    \label{tab:example}
\end{table}

==> table/exp_result.tex <==


\begin{table*}[h!]
    \centering
    \setlength{\tabcolsep}{2pt}
    \caption{experiment result}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{c|c|cccc|cccc|cccc|c|cccc|cccc|cccc|c|cccc|cccc|cccc|c|c}
            \hline
            & & \multicolumn{13}{c|}{\textbf{Customization}} & \multicolumn{13}{c|}{\textbf{Contextualization}} & \multicolumn{13}{c|}{\textbf{Stylization}} & 
            \\
            % \cline{2-42}
            \hline
            
            & \multicolumn{1}{c|}{Dimension} 
            & \multicolumn{4}{c|}{\makecell{Derivative Character}} & \multicolumn{4}{c|}{\makecell{Reimagined Representations}} & \multicolumn{4}{c|}{\makecell{Surreal Fantasy}} & \multicolumn{1}{c|}{Average}
            & \multicolumn{4}{c|}{\makecell{Artistic Style \\ Transformation}} & \multicolumn{4}{c|}{\makecell{Identity\&Cultural \\ Transformation}} & \multicolumn{4}{c|}{Material Transformation} & \multicolumn{1}{c|}{Average}
            & \multicolumn{4}{c|}{\makecell{Containerized \\ Scenario}} & \multicolumn{4}{c|}{\makecell{Commercial \\ Design}} & \multicolumn{4}{c|}{\makecell{Informationization\& \\ Narrative Expression}} & \multicolumn{1}{c|}{Average}
            & \multicolumn{1}{c}{\textbf{\makecell{Overall \\ Average}}} 
            \\
            
            % \cline{2-42}
            \hline
            & Metric & IF & VC & VQ & avg & IF & VC & VQ & avg & IF & VC & VQ & avg & -
            & IF & VC & VQ & avg & IF & VC & VQ & avg & IF & VC & VQ & avg & -
            & IF & VC & VQ & avg & IF & VC & VQ & avg & IF & VC & VQ & avg & - & -
            \\
            
            \hline
            \multirow{3}{*}{\rotatebox{90}{\textbf{\textit{Close-Source Models}}}}
            & Bagel & 88.88 & 88.88 & 88.88 & 88.88 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 88.88 & 88.88 & 88.88 & 88.88 & 88.88 & 88.88 & 88.88 & 88.88 & 00.00 & 00.99 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.0 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
            & Bagel-think & 00.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
            & OmniGen2 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
            & Qwen-image-Edit &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
            & FLUX.1 Kontext[dev]  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
            
            \hline
            \multirow{1}{*}{\rotatebox{90}{\textbf{\textit{Open-Source Models}}}}
            & GPT &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
            & seedream4.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
            & Gemini 2.5 Flash Image (Nano Banana) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
            
            \hline
            \end{tabular}
        }
        
    \label{tab:example}
\end{table*}

==> table/open-source-models.tex <==
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.1}
    \caption{experiment result}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c|c|ccccccccc}
            \noalign{\hrule height 1.5pt}
            
            \multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Dimension}} & \multirow{2}{*}{\textbf{Metric}} & 
            \multicolumn{9}{c}{\textbf{Open-source Models}} \\
            \cline{4-12}

            & & &
             \textbf{OmniGen2} &\textbf{Bagel} & \textbf{Bagel(think)} & \textbf{UniWorld-V1} & \textbf{ICEdit} & \textbf{Qwen-Image-Edit} & \textbf{FLUX.1 Kontext[dev]} & \textbf{Step1X-Edit-v1p2-preview} & \textbf{Step1X-Edit-v1p2-preview (think)} 
            \\
            \hline
            

            \multirow{13}{*}{\rotatebox{90}{\textbf{Customization}}} 
            & \multirow{4}{*}{\makecell{Derivative \\ Character}} & IF & 88.88 & 00.00 &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VC & 88.88 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VQ & 88.88 &  &  &  &  &  &  &  &    \\
            % \cline{3-11}
            & & avg & 88.88 &  &  &  &  &  &  &  &    \\
            \cline{2-12}
            
            & \multirow{4}{*}{\makecell{Reimagined \\ Representations}} & IF & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VC & 00.00 &  &  &  &  &  &  &  &    \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & avg & 00.00 &  &  &  &  &  &  &  &     \\
            \cline{2-12}
            
            & \multirow{4}{*}{\makecell{Surreal \\ Fantasy}} & IF & 00.00 &  &  &  &  &  &  &  &    \\
            % \cline{3-11}
            & & VC & 88.88 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VQ & 88.88 &  &  &  &  &  &  &  &      \\
            % \cline{3-11}
            & & avg & 88.88 &  &  &  &  &  &  &  &      \\
            \cline{2-12}
            
            & \textbf{Average} & - & 88.88 &  &  &  &  &  &  &  &     \\
            % \hline
            \noalign{\hrule height 1.5pt}
            
            
            % Contextualization任务组
            \multirow{13}{*}{\rotatebox{90}{\textbf{Contextualization}}} 
            & \multirow{4}{*}{\makecell{Containerized \\ scenario}} & IF & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VC & 00.00 &  & &   &  &  &  &  &     \\
            % \cline{3-11}
            & & VQ & 00.00 &  & & & &  &  &  &     \\
            % \cline{3-11}
            & & avg & 00.00 &  & & & &  &  &  &     \\
            \cline{2-12}
            
            & \multirow{4}{*}{\makecell{Commercial \\ design}} & IF & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VC & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & avg & 00.00 &  &  &  &  &  &  &  &     \\
            \cline{2-12}
            
            & \multirow{4}{*}{\makecell{Informationization\& \\ Narrative Expression}} & IF & 00.00 &  & &  &  &   &  &  &  \\
            % \cline{3-11}
            & & VC & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & avg & 00.00 &  &  &  &  &  &  &  &     \\
            \cline{2-12}
            
            & \textbf{Average} & - & 00.00 &  & &  &  &  &  &  &     \\
            \noalign{\hrule height 1.5pt}
            
            % Stylization
            \multirow{13}{*}{\rotatebox{90}{\textbf{Stylization}}} 
            & \multirow{4}{*}{\makecell{Artistic Style \\ Transformation}} & IF & 88.88 &  & &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VC & 88.88 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VQ & 88.88 &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & avg & 88.88 &  &  &  &  &  &  &    \\
            \cline{2-12}
            
            & \multirow{4}{*}{\makecell{Identity\&Cultural \\ Transformation}} & IF & 00.00 &  & &  &  &  &  &  &   \\
            % \cline{3-11}
            & & VC & 00.99 &  &  &  &  &  &  &  &      \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & avg & 00.00 &  &  &  &  &  &  &  &     \\
            \cline{2-12}
            
            & \multirow{4}{*}{\makecell{Material \\ Transformation}} & IF & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VC & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & VQ & 00.00 &  &  &  &  &  &  &  &     \\
            % \cline{3-11}
            & & avg & 00.00 &  &  &  &  &  &  &  &     \\
            \cline{2-12}

            & \textbf{Average} & - & 00.00 &  & &  &  &   &  &  &   \\
            \hline
            
            & \multicolumn{2}{c|}{\textbf{Overall Average}} & 00.00 &  &  &  &  &  &  &  &   \\
            \noalign{\hrule height 1.5pt}
        \end{tabular}
    }
    \label{tab:example}
\end{table*}
